Entropy Estimation via Uniformization

Entropy estimation is of practical importance in information theory and statistical science. Many existing entropy estimators suffer from fast growing estimation bias with respect to dimensionality, rendering them unsuitable for high-dimensional problems. In this work we propose a transform-based method for high-dimensional entropy estimation, which consists of the following two main ingredients. First by modifying the k-NN based entropy estimator, we propose a new estimator which enjoys small estimation bias for samples that are close to a uniform distribution. Second we design a normalizing flow based mapping that pushes samples toward a uniform distribution, and the relation between the entropy of the original samples and the transformed ones is also derived. As a result the entropy of a given set of samples is estimated by first transforming them toward a uniform distribution and then applying the proposed estimator to the transformed samples. The performance of the proposed method is compared against several existing entropy estimators, with both mathematical examples and real-world applications.

==> response_to_reviewers.tex <==
REVIEWERS' COMMENTS:

Associate Editor: I agree with the reviewers that this paper is novel in technical content and deserves to be published at AIJ. However, the current manuscript is (almost) a direct submission of the conference paper (with some new materials and correction of typos), and most of the sentences are identical. To qualify as a "new" journal paper, the authors should thoroughly revise the writing and further improve the readibility.

A：We have made substantial revision and extension in the new manuscript, which makes it considerably different from the conference version.
The main extensions  in the first version of the journal submission:
1. We extended the original Corollary 2 to Corollaries 2 & 3 in the revised paper, which further analyzes the MSE of the UM based estimators.
2.	We added Algorithm 1 that summarizes the construction of estimator (13).
3.	We added details of how to naturally use the framework of NF to construct UM in Section 3.3 (see p14, l11 to p15 l6).

Further extensions made in the revised version: 
4.	We significant revised the abstract and the introduction section. In particular we included a more comprehensive literature review in the introduction, with some up-to-date work added (see p2 l30-36).
5.	We expanded the Numerical Experiments section into two: Numerical Experiments and Application Examples.
    5.a)	In the Numerical Experiments section (i.e. Section 4), we added two more experiments. In Section 4.1, we provided an illustrating example for the truncated estimators. In section 4.4, we used a modified Rosenbrock distributions which have discontinuous densities to validate the methods when the assumption of differentiability is not satisfied.
    5.b)   In Section 5, we added a new application example, which is the entropy rate estimation of time series signals.
6.  In the Conclusion section,  we added discussions on several future research directions. 
7. As suggested by Reviewer #1, we included the skeleton proofs for the two main theorems (Thm 1 and 2) in the main text, which provide a roadmap for
the complete proof detailed in the Appendix.

Reviewer #1: 
The biggest part the reviewer would complain about is the
readability of the proof. If the authors want to publish their paper in a
journal which always has a sufficient page budget, I believe more work needs to
be done...

A: Following the reviewer's suggestion, we have included skeleton proofs for the two main theorems (Thm 1 and 2) in the main text, which provide a roadmap for the complete proof detailed in the Appendix. 

There are also a few additional minor comments:

Figure 1 does not seem to be referenced and explained anywhere in this paper.
 A: Corrected and it is referenced to in (p7, l0). 

Algorithm 1 can be improved using standard algorithm formate. The bullet points
are normally unordered, while programs normally are executed sequentially.

A: we changed to numbered items. 

In Proposition 2, \pi does not seem well defined anywhere in this paper.
  A: We added explanation of distribution $\pi$ in the statement of the proposition.

In line 210, the multivariate beta distribution B(b,b) should be B(b,d) or B(d,b).
  A: In general the beta distributions has two independent parameters $b$ and $d$. Here we assume the two parameters are identical, i.e. $b=d$.

Reviewer #2: 


- In paragraph 120, "the SI" should be Section 4.1.
- The line break on Eq. (11) appears unnecessary.

A: We corrected the typos.

Reviewer #3: 

In addition, I have the following questions and suggestions：
1. The method proposed in the paper is a better estimation of entropy, why "RMSE" is used as the main evaluation metric in the experimental part instead of entropy value itself as in the comparison work [1]?
A: We understand that in [1], the average absolute error (which essentially is the estimation bias) is used in [1], because the authors of [1] obtained an analytical bound (Section 3.2 in [1]) for such an error and wanted to compare it against the numerical results. On the other hand, RMSE consists of both the variance and the bias, and therefore is more informative. We have found it is used in many existing works, e..g [25] in the manuscript.  

2. For the completeness of the experiment, I think it is better to add "UM_KL" and "UM_KSG" for the ablation experiment.
A: We think essentially the reviewer wants to see how KL/KSG compared against tKL/tKSG.
In the revised draft, we proposed to address the issue by adding Section 4.1, in which we applied both KL/KSG and tKL/tKSG to distributions with compact support (recall that after UM, the distributions are compactly supported). The numerical results given in this section shows that the truncated estimators have evidently better performance.   

3. The explanation of Proposition 2 is not clear enough. The meaning of distribution $\pai$ is not described.
A: We added explanation of distribution $\pi$ in the statement of the proposition.

4. All numerical experimental results are based on the simulated data, is it possible to test in some real world scenarios?
A: The main purpose of the present paper is to propose the entropy estimation method and examine its performance, and as such we chose to use simulated data so that we can easily validate the outputs of the method and evaluate its performance. That said, we provided two application examples (a new one added in the revised draft) to (at least partially) demonstrate our method's performance in such real-world scenarios. We acknowledge that in the application examples 
we still used the simulated data, and we plan to apply the method to real-world data sets in application-focused projects. We added such a discussion in the Conclusion.   

5. A minor issue: "RMSE" first appears in line 216 instead of line 232.
  A: We corrected the issue.
  
Ref:
[1].G. Ariel, Y. Louzoun, Estimating differential entropy using recursive copula splitting, Entropy 22 (2) (2020) 236.






